Solid Geometry Processing on Deconstructed Domains

Many tasks in geometry processing are modeled as variational problems solved numerically using the finite element method. For solid shapes, this requires a volumetric discretization, such as a boundary conforming tetrahedral mesh. Unfortunately, tetrahedral meshing remains an open challenge and existing methods either struggle to conform to complex boundary surfaces or require manual intervention to prevent failure. Rather than create a single volumetric mesh for the entire shape, we advocate for solid geometry processing on deconstructed domains, where a large and complex shape is composed of overlapping solid subdomains. As each smaller and simpler part is now easier to tetrahedralize, the question becomes how to account for overlaps during problem modeling and how to couple solutions on each subdomain together algebraically. We explore how and why previous coupling methods fail, and propose a method that couples solid domains only along their boundary surfaces. We demonstrate the superiority of this method through empirical convergence tests and qualitative applications to solid geometry processing on a variety of popular second-order and fourth-order partial differential equations.

==> 1d.tex <==
\section{One dimension}
\label{sec:one-dimension}

We start our derivations in the smooth setting and with a simple one
dimensional Poisson problem. 
\alec{Start dimension agnostic, instead}
We would like to find a function $u(s)$ that minimizes
its squared first derivative plus a uniform load over the unit line segment
$s ∈ Ω := [0,1] ⊂ \R$ subject to prescribed values $f_0,f_1$ at the segment
boundaries:
\begin{align}
\label{equ:1d-original-poisson-energy}
\min_u       & ∫_Ω \underbrace{\left(½ ‖u'‖² + u\right)}_{E(u)} \ds \\
\text{subject to } & u(0)=f_0 \text{ and } u(1)=f_1,
\end{align}
where $E(u)$ measures the local energy density at some point $s$ in the
domain.

Calculus of Variations reveals that the minimizer corresponds to the solution to
the second-order partial differential equation, the 1D Poisson equation:
\begin{equation}
%
\label{equ:1d-original-poisson-equation}
%
u''(s) = -1 \ \text{ for $s∈Ω$, subject to $u(0)=f_0$ and $u(1)=f_1$}.
\end{equation}
Discrete approximations to such second-order PDEs can be readily computed using
finite element method using a piecewise-linear discretization of the unit line
segment
(see \reffig{1d-poisson}).

For the sake of progressing this example, suppose that we are incapable of
discretizing the unit segment directly, and instead we must consider it only as
the union of two smaller, overlapping segments: $Ω₁ := [0,⅔]$ and $Ω₂ := [⅓,1]$.
In the smooth setting, we can quickly verify that finding the optimal function
$u$ over $Ω$ in \refequ{1d-original-poisson-energy} is equivalent to finding the
functions the functions $u₁$ and $u₂$ over $Ω₁$ and $Ω₂$ that minimize the
combined energy subject to equality constraints forcing equality between $u₁$
and $u₂$ in the shared intersection region $Ω₁ ∩ Ω₂$:

\begin{align}
%
\label{equ:1d-deconstructed-energy}
%
\min_{u₁,u₂} & 
    ∫_{Ω₁ \setminus Ω₂ } E(u₁) \ds +  ∫_{Ω₂ \setminus Ω₁ } E(u₂) \ds + \\
\label{equ:1d-deconstructed-energy-intersection-term}
                     & ½∫_{Ω₁∩Ω₂} \left(E(u₁) + E(u₂)\right) \ds \\
  \text{subject to } & u₁(0) = f_0 \text{ and } u₂(1) = f_1, \\
\label{equ:1d-deconstructed-energy-equality-constraint}
  \text{       and } & u₁(s) = u₂(s) \ ∀ s ∈ Ω₁∩Ω₂.
\end{align}

To sketch a proof of equivalence, we note that both the original energy in
\refequ{1d-original-poisson-equation} and the 
deconstructed energy in \refequ{1d-deconstructed-energy} are a strictly convex,
each with a unique global minimum.
%
Let us define a new function $v$ over the
original unit segment $Ω$ so that it takes on values of given
minimizers $u₁$ and $u₂$ on their respective sub-domains:
\begin{equation}
  \label{equ:combined-function}
  v(s) = \begin{cases} u₁(s) & s∈Ω₁ \\ u₂(s) & s∈Ω₂ \end{cases}.
\end{equation}
%
The measured energy of $u₁$ and $u₂$ in \refequ{1d-deconstructed-energy} is
equal to the measured energy of $v$ in \refequ{1d-original-poisson-energy}. By
uniqueness, $v$ must be equal to the minimizing $u$ to the original problem.

\paragraph{Advantage of working with energies}
%
The factor of $½$ appearing before the integrated energy in the intersection $Ω₁
∩ Ω₂$ region (see \refequ{1d-deconstructed-energy-intersection-term}) would not
be so obvious if we had 
worked with the Poisson problem directly as a PDE (see
\refequ{1d-original-poisson-equation}).
%
However, viewed as an energy minimization, the necessity of the $½$ is clear:
if we split $u$ into two functions we should not double count the energy
contributed in this region.

Moving to the discrete setting, let us assume that we discretize both $u₁$ and $u₂$ using
piecewise-linear finite elements:
\begin{align}
  \begin{array}{cc}
  u₁ = \sum\limits_{i=1}^{n₁} u_1^i φ₁^i(s),
  & u₂ = \sum\limits_{j=1}^{n₂} u_2^j φ₂^j(s),
  \end{array}
\end{align}
using the notation where $u_1^i$ is the interpolated value at the $i$th vertex
of the mesh with $n₁$ vertices covering subdomain $Ω₁$ and $φ₁^i$ is the typical
piecewise linear hat function centered there.

\subsection{\alec{Locking}}
Discretizing the constraint in
\refequ{1d-deconstructed-energy-equality-constraint} as \emph{point-wise}
equality in the intersection region $Ω₁∩Ω₂$ will restrict the search space to
piecewise linear functions that exist mutually in both linear FEM function
spaces. 

If the meshes over $Ω₁$ and $Ω₂$ have only and exactly co-incident vertices (and
compatible combinatorics) in the intersection region $Ω₁∩Ω₂$, then we call them
\emph{matching} then point-wise equality is equivalent to merging the meshes:
the search space is as rich as linear FEM over the merged mesh and no locking
occurs.

When meshes are in general position, perfect coincidence never happens.
%
The constrained space reduces dramatically: \emph{only} functions that take on a
linear function over $Ω₁∩ Ω₂$ are left (see \reffig{1d-poisson}).

This is an extreme case of what is known as \emph{locking} in the finite element
literature \alec{cite a book}. Locking is an artificial stiffening of system
during discretization. In our case, the constraints have stiffened the system so
much that only rather boring functions remain. These functions can be
arbitrarily far from the desired solution and discretization refinement by
adding more vertices (in general position) will not help (see
\reffig{1d-poisson}).

One strategy (e.g., \alec{not quite: } \cite{KozlovBBTBG17}) is to require equality only at mesh
vertices. This ties the values at one mesh's vertices to the piecewise linearly
interpolated value on the other mesh via a linear equality constraint and
\emph{vice-versa}, e.g.,:
\begin{align}
  \label{equ:naive-constraints}
  u_1^i &= \sum\limits_{j=1}^{n₂} u_2^j φ₂^j(s_1^i), 
    \ \text{for any} \ i \text{ such that } s_1^i ∈ Ω₁∩Ω₂, \\
  u_2^j &= \sum\limits_{i=1}^{n₂} u_1^i φ₁^i(s_1^j), 
    \ \text{for any} \ j \text{ such that } s_2^j ∈ Ω₁∩Ω₂,
\end{align}
where $s_1^i$ is the position of the $i$th vertex in the mesh over subdomain
$Ω₁$. This constraint is easy to implement in practice (e.g., via the null space
or Lagrange multiplier method), but unfortunately do not alleviate locking.

\subsubsection{\alec{1D linear locking}}
%
Intuitively, if a segment of the mesh over $Ω₁$ overlaps with a segment of the
mesh over $Ω₂$ then both pairs of vertices will have to lie on the same line. In
the worst case of alternating order of vertices from $Ω₁$ and $Ω₂$, this will
have a Domino effect and the entire intersection region locks to the same linear
function (see \reffig{1d-domino-effect}).

We will differ our discussion and comparison to other \emph{ad hoc} softenings
of this equality constraint to \refsec{experiments} and instead return to the
smooth setting to derive a locking-free solution from first principles.

\subsection{Boundary-only constraints}
%
Point-wise equality over the entire intersection region (see
\refequ{1d-deconstructed-energy-intersection-term}) is redundant \cite{schwarz}.
It suffices to require equality \emph{only along the boundary of the
intersection of the overlapping regions}:
%
\alec{This is stated too matter of factly. This is supposed to be the punchline
of the paper.}
%
\begin{equation}
  \label{equ:1d-deconstructed-energy-boundary-only-constraint}
  u₁(s) = u₂(s) \ ∀ s ∈ ∂(Ω₁∩Ω₂).
\end{equation}

Proof of equivalence follows similarly \alec{similarly to what?}.
\silvia{Similarly to the proof sketched in the previous page regarding the
'naive' conditions. See after eq. (7)}
The problem in
\refequ{1d-deconstructed-energy} replacing the point-wise constraint
\refequ{1d-deconstructed-energy-equality-constraint} with the boundary-only
constraint \refequ{1d-deconstructed-energy-boundary-only-constraint} remains
convex with a unique minimizer. The function $u₁$ satisfies the Poisson
equation $u₁'' = -1$ over $Ω₁$, likewise $u₂'' = -1$ over $Ω₂$. Therefore the
function $v$ (as defined in \refequ{combined-function}) satisfies this Poisson
equation $v'' = -1$ over all of $Ω$. By uniqueness, it must be equal to the
minimizer of the original problem \refequ{1d-original-poisson-energy}.

Returning to the discrete setting, we now allow our piecewise linear
discretizations of $u₁$ and $u₂$ to \emph{disagree} in the intersection region
$Ω₁ ∩ Ω₂$, only requiring that $u₁$ equal to the value of the piecewise linear
function $u₂$ at the boundary \emph{vertex} at $s=⅔$ (and similarly for $u₂$'s
vertex at $s=⅓$):
%
\begin{align}
  u_1^i &= \sum\limits_{j=1}^{n₂} u_2^j φ₂^j(s_1^i), 
    \ \text{for any} \ i \text{ such that } s_1^i ∈ ∂(Ω₁∩Ω₂), \\
  u_2^j &= \sum\limits_{i=1}^{n₂} u_1^i φ₁^i(s_1^j), 
    \ \text{for any} \ j \text{ such that } s_2^j ∈ ∂(Ω₁∩Ω₂),
\end{align}
keeping in mind that a vertex at position $s_1^i$ lying along the boundary of
the subdomain $Ω₁$ will -- in general -- lie in the interior of some element of
the subdomain $Ω₂$.

\alec{yuck. We might have to explicitly write out the linear FEM discretization
of $u₁$ and $u₂$ and spell out this constraint. It'd be great if we could
postpone this until \refsec{higher-dimensions}.}
\silvia{A way to avoid that might be to, instead of calling things ``piecewise
linear'' and using FEM language at this point, we can merely say this is a
discrete function where the value between vertices is linearly interpolated.
This is simple, understandable and does not require to write things explicitely.
We can always add in the next section, once we explicitely write the FEM
discretization, something like ``note that the process described for 1D meshes
is equivalent to the one described here''.}
\alec{I don't quite see how it would help yet.}

For any point in the intersection region $s ∈ Ω₁ ∩ Ω₂$, we now have two possible
values $u₁(s)$ and $u₂(s)$ that in general do not agree, though they both
converge to the true solution under refinement (see \reffig{1d-poisson}):
implying that their difference also vanishes. Locking does not occur.

\alec{In 1D the boundary of a segment domain are just the endpoint vertices. For
higher dimensions, there are boundary poly-curves/-surfaces. Constraining
equality pointwise would similarly result in linear locking inside elements
overlapping the boundary of another domain. Thus, constraints are applied at
boundary vertices only.}
\silvia{Shouldn't this go in sec. 4.2? I can write it down if you wish, it's not
in the to-do list.}

\alec{hopefully remove this. These ``generalizations'' are not really the
contribution, except the higher-order thing but it's getting burried in this
list.}
We now generalize from this simple Poisson problem over the 1D union of two
segments in a variety of ways. We generalize in dimension to 2D triangle meshes
and 3D tetrahedral meshes. We generalize the union to arbitrary constructive
solid geometry operations, including intersection and differencing. Finally, we
generalize to other energy minimization and partial differential equations,
including fourth-order partial differential equations.



==> acks.tex <==
remember to cite Barill:2018 in conclusion

Eitan
Dave
Fields Institute
Tomograph
Oded
Silvia's scholarship

Proofreading
Gavin
Sarah
Darren
M Tao


==> biharmonic.tex <==
\section{Higher-order Partial Differential Equations}
\label{sec:biharmonic}



==> ccsxml.tex <==
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002950.10003714.10003715.10003750</concept_id>
<concept_desc>Mathematics of computing~Discretization</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10002950.10003714.10003727.10003729</concept_id>
<concept_desc>Mathematics of computing~Partial differential equations</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10002950.10003714.10003715.10003724</concept_id>
<concept_desc>Mathematics of computing~Numerical differentiation</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010371.10010352</concept_id>
<concept_desc>Computing methodologies~Animation</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010371.10010396.10010398</concept_id>
<concept_desc>Computing methodologies~Mesh geometry models</concept_desc>
<concept_significance>300</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Mathematics of computing~Discretization}
\ccsdesc[500]{Mathematics of computing~Partial differential equations}
\ccsdesc[300]{Mathematics of computing~Numerical differentiation}
\ccsdesc[300]{Computing methodologies~Animation}
\ccsdesc[300]{Computing methodologies~Mesh geometry models}

\keywords{Geometry processing, smoothing, denoising, Hessian energy, Laplacian energy}



==> csg.tex <==
\section{Constructive solid geometry}
\label{sec:csg}


==> discrete.tex <==
\section{Discrete setting}
\label{sec:discrete}
 
- point location

- barycentric coordinates

- linear FEM
\silvia{do you plan on going all through FEM and mixed FEM or just citing some
paper and starting with the corresponding matrices?}
\alec{just a citation}

- higher order: mixed FEM

\begin{figure}
%\includegraphics[width=\linewidth]{figs/omega-deconstruction}
\caption{\label{fig:2d-annulus-laplace-poisson}
Convergence plot for Dirichlet vs. Naive vs. co-refine for Laplace and Poisson
equation in 2d.}
\end{figure}

\begin{figure}
%\includegraphics[width=\linewidth]{figs/omega-deconstruction}
\caption{\label{fig:3d-annulus-laplace-poisson}
Convergence plot for Dirichlet vs. Naive vs. co-refine for Laplace and Poisson
equation in 3d.}
\end{figure}

\begin{figure}
%\includegraphics[width=\linewidth]{figs/omega-deconstruction}
\caption{\label{fig:3d-annulus-bilaplace}
Convergence plot for Dirichlet vs. Naive vs. co-refine for bilaplace 
  \silvia{and bipoisson?}
  \alec{BiLaplace should already be interesting, no?}
equation in 3d.}
\end{figure}

- CSG: generalization

- CSG: regularization in ``exterior'' regions



==> higher-dimensions.tex <==
\section{Higher dimensions}
\label{sec:higher-dimensions}

We may extend our discussion and derivations from 1D to higher dimensions. For
example, in 2D the intersection region $Ω₁ ∩ Ω₂$ becomes a 2D area with a 1D
curve boundary. We may use triangle meshes with analogous piecewise linear hat
functions $φ_i$ interpolating values at vertices to discretize each function
$u_i$ over its corresponding subdomain $Ω_i$.

Assuming general position, pointwise equality (see
\refequ{1d-deconstructed-energy-equality-constraint}) over the entire 2D
intersection region will still result in locking to a single linear function.


Constraining to equality at \emph{all} vertices in the intersection region in 2D
(cf.\ \refequ{naive-constraints}) also results in a form of locking, but --
somewhat surprisingly -- the search space is not limited to just linear
functions. 

We now analyze this case in more detail. The categorization of the
space leads to an interesting connection to discrete differential geometry, but
ultimately the space is too limited for practical use. Thus, necessitating the
need for boundary-only constraints (cf.\
\refequ{1d-deconstructed-energy-boundary-only-constraint}) in higher dimensions.

\subsection{Harmonic locking}
\label{sec:harmonic-locking}
%
The first phenomenon we observe is that constraining all intersection vertices
in 2D shapes returns promising results when attempting to solve the Laplace
equation $\Delta u = 0$. The solutions to these equations (known as harmonic
functions) are generally saddle-shaped with negative Gaussian curvature. When we
move on, however, and consider the Poisson equation $\Delta u = g$ with non-zero
right-hand side (which results in a solution with positive curvature),
constraining all vertices shows itself to be a failure (see
\reffig{saddle-vs-parabola}).


\wf{}{l}{0.75in}{trim={0mm 0mm 5mm 1mm},width=0.75in}{figs/harmonic-didactic}{}
%
A comparative modal analysis of these linear constraints and the discrete
Laplacian shown in \reffig{eigen-modes} immediately determines that this is not a coincidence . In
fact, the more regular the meshes are and the more 'general' their relative
position is, the closer our constraint matrix is to the linear cotangent
Laplacian (see inset). Hence, by applying this constraint to the function space
we are actually
enforcing a sort of \emph{harmonic locking}. The linear locking we experienced
in 1D can now also be seen as a form of harmonic locking given that the only
one-dimensional harmonic functions are precisely the linear ones.

Furthermore, it can be proven that if these
constraints are enforced, the value of the energy minimizer on the intersection
is uniquely determined (assuming general position) by the value on its boundary,
meaning that it will generally hold no relation to the energy being minimized.
Therefore, while harmonic locking is certainly a step in the right direction from its
linear counterpart, it remains catastrophic for many problems whose solutions
are not harmonic: Poisson equations (see \reffig{2d-annulus-convergence}),
Bi-Laplace/-Poisson equations, etc. This undesirable effect caused by
constraining all intersection vertices moves us to consider
boundary-only constraints much like
we did in the one-dimensional case.
%- harmonic functions -- boring in 1D -- are interesting in 2d, we might expect
%"linear locking", but we actually observe "harmonic locking". why? regular grid
%C'C  = graph Laplacian

\alec{cite something from ``curvature theory'' lit. Wardetzky/Hoffman/Walner}

%The linear locking in 1D can now be understood also as harmonic locking: in 1D,
%the only harmonic functions ($u'' = 0$) are the linear functions.
%
%Not surprisingly, harmonic locking is not so disastrous when the underlying
%solution is itself a harmonic function (see
%\reffig{2d-annulus-laplace-poisson}).
%
%... despite this gift of freedom compared to complete linear locking, harmonic
%locking is still catastrophic for many problems whose solutions are not
%harmonic: Poisson equations (see \reffig{2d-annulus-laplace-poisson}),
%Bi-Laplace/-Poisson equations, etc. 

\subsection{Boundary-only constraints in higher dimensions}

- only require constraints at vertices, not point-wise on boundary

\subsection{Multiple subdomains}

In 2D, we also see the possibility to cover a domain $Ω$ with a union of $m>2$
subdomains where more than two domains overlap at some places.

When transferring a problem over the entire domain $Ω$ such as the Poisson
problem in \refequ{1d-original-poisson-energy}
%
We must adjust for more general multiplicity, generalizing the introduction of
the $½$ in 
\refequ{1d-deconstructed-energy} to a fraction whose denominator counts
the number of subdomains any positions $\s$ is inside:
%
\begin{align}
\label{equ:deconstructed-energy}
  ∫_{Ω} E(u) \;d\s    &= ∫_{Ω} \frac{1}{∑_{i=1}^m χ_i} E(u) \;d\s \\
  \text{where } χ_i(\s) &= 
    \begin{cases} 
      1 & \text{ if } \s ∈ Ω_i, \\ 
      0 & \text{ otherwise,}
    \end{cases}
\end{align}
defining $χ_i$ to be the characteristic (a.k.a., indicator) function of $Ω_i$.
%

\paragraph{Quadrature/cut-cell}
%
This fractional re-weighting effectively scales the \emph{density} during
integration.
%
The weighting function
$\frac{1}{∑_{i=1}^m χ_i}$ will be piecewise constant (cf.\ the PWN meshes of
\cite{Zhou2017}).
%
During discretization with a triangle mesh, the function may take on different
values within a single triangle lying across other subdomain boundaries.
\alec{Small wrapfig here.}
%
Performing geometric mesh surgery to subdivide triangle along other boundaries
so that the weight function is constant within every triangle is theoretically
possible, but we immediately inherit all the original problems with conforming
meshing. These problems are much more extreme in 3D.

Instead, we experimented with various approximations common to cut-cell methods
in simulation (\cite{Batty}).

- random vertex 

- winner takes all, vertex voting

- barycenter (1st order quadrature)

- higher order quadrature (e.g., 8th order or something ``big'')

\paragraph{Avoiding constraint redundancy}


The immediate way of generalizing our boundary-only constraints to the overlap
of more than two domains is to proceed pair-wise, i.e. to build all of the
boundary-only constraints for each possible pair of domains. In the case where
the boundaries of more than two shapes intersect, this will intuitively lead to
a redundancy of constraints which results in locking
(\reffig{4-spheres-geodesics-in-heat}). While rare in 2D shapes, this
topological phenomenon is very common in three-dimensional intersecting shapes,
making this type of near-linear locking a very significant problem.

The optimal way of resolving this issue would be to keep the minimum amount of
constraints such that the maximum amount of the intersection's boundary vertices
are affected by them. The obvious similarity between this and the classic
maximum coverage problem \silvia{do we need a citation here?} (which is known to
be NP-hard) will motivate us not to search for the optimum subset of constraints
described above but to be content with an approximation.

\silvia{Here's the thing, I think we should ellaborate on the approximation,
much like we do in the figure's caption. But having the explanation both in the
main text and the caption seems redundant. What are your thoughts? I would
shorten the caption and add here details on precisely how the approximation is
made.}



==> smooth.tex <==
\section{Smooth setting}
\label{sec:smooth}

\alec{I'm not sure this smooth-then-discrete organization is right. It will be
awkward to bring up  ``locking'' without yet describing discretization.}


We start our derivations in the smooth setting. Let us initially consider the
following Dirichelt problem. We would like to find a function $u$ 
that minimizes its integrated
squared gradient
over a solid
domain $Ω ⊆ \R^2$ (or analogously $Ω ⊆ \R^3$) subject to prescribed 
values $f$ on the domain boundary $∂Ω$:
$$
u^* = \argmin_u ∫_Ω ‖∇u‖² \dA \ \text{ subject to $u=f$ on $∂Ω$}.
$$
\silvia{Is there any reason to restrict to the zero rhs case?}
\alec{I'm not entirely sure of the organization of this part of the paper yet,
but the intention is to start with a simple example.}

\begin{figure}
\includegraphics[width=\linewidth]{figs/omega-deconstruction}
\caption{\label{fig:omega}
A solid domain is deconstructed as the union of three smaller, simpler domains:
$Ω = Ω₁ ∪ Ω₂ ∪ Ω₃$.}
\end{figure}

Now, assume that that we are not given $Ω$ directly, but rather a set of $n$
smaller, solid subregions $Ω_i ⊂ Ω$ so that their union is exactly the intended
domain $Ω$ (see \reffig{omega}):
$$
Ω =  Ω₁ ∪ Ω₂ ∪ … ∪ Ω_n.
$$
We will restrict ourselves to working with functions $u_i$ defined on each
subdomain $Ω_i$.

\silvia{Again, why restrict to unions? Why not "imagine $\Omega$ is constructed
as some set function on $n$ simple domains $\Omega_i$." We can even change the
next paragraph to ``...two subdomains, $\Omega_1$ and $\Omega_2$ and $\Omega =
\Omega_1\cup\Omega_2$. Our first...''. We can afterwards show what happens for
set substractions, which contains all other set operations.}
\alec{too general too soon. this will eventually come later as a modification of
this simpler case.}

For now, let us assume we have just two subdomains ($n=2$). Our first
observation is that we 

- must not double count area

- proof of naive constraints

- proof of boundary-only Dirichlet constraint 

- counterexample to Neumann boundary conditions (annulus)

\begin{figure}
%\includegraphics[width=\linewidth]{figs/omega-deconstruction}
\caption{\label{fig:double-count-area}
Figure showing that we must not double-count energy in intersection.}
\end{figure}

\begin{figure}
%\includegraphics[width=\linewidth]{figs/omega-deconstruction}
\caption{\label{fig:1d}
Figure showing 1d simple solution, 1d naive constraints locking, 1d Dirichelt
success, 1d Neumann fail}
\end{figure}



==> suggestion.tex <==
\section{An example: union of two domains}
We start our derivations in the smooth setting. Let us initially consider the
following Dirichelt problem. We would like to find a function $u$ 
that minimizes its integrated
squared gradient
over a solid
domain $Ω ⊆ \R^2$ (or analogously $Ω ⊆ \R^3$) subject to prescribed 
values $f$ on the domain boundary $∂Ω$:
$$
u^* = \argmin_u ∫_Ω ‖∇u‖² \dA \ \text{ subject to $u=f$ on $∂Ω$}.
$$
